Understanding Generalization in Deep Learning via Tensor Methods

Deep neural networks generalize well on unseen data though the number of parameters often far exceeds the number of training examples. Recently proposed complexity measures have provided insights to understanding the generalizability in neural networks from perspectives of PAC-Bayes, robustness, overparametrization, compression and so on. In this work, we advance the understanding of the relations between the network's architecture and its generalizability from the compression perspective. Using tensor analysis, we propose a series of intuitive, data-dependent and easily-measurable properties that tightly characterize the compressibility and generalizability of neural networks; thus, in practice, our generalization bound outperforms the previous compression-based ones, especially for neural networks using tensors as their weight kernels (e.g. CNNs). Moreover, these intuitive measurements provide further insights into designing neural network architectures with properties favorable for better/guaranteed generalizability. Our experimental results demonstrate that through the proposed measurable properties, our generalization error bound matches the trend of the test error well. Our theoretical analysis further provides justifications for the empirical success and limitations of some widely-used tensor-based compression approaches. We also discover the improvements to the compressibility and robustness of current neural networks when incorporating tensor operations via our proposed layer-wise structure.

==> 1.1_setup.tex <==
\subsection{Generalization with Tensor Methods}
The theoretical analyses in~\citep{arora2018stronger} connect the generalizability of a neural network to its compressibility. In this work, we show how tensor methods can provide further insight into the understanding of this connection. We propose a series of measures to study the properties of such decomposed networks. 

In our theoretical analysis, we present a rigorous proof showing the connection of these factors to the generalization error of a network. We will see in experiment section that this calculated bound is very effective at predicting the generalization error after some proper rescaling. 

Although our theoretical analysis is derived for neural networks with \ourNN, our proposed generalization bounds are extended to any fully connected neural network (Theorem~\ref{thm:main_thm}), convolutional neural network (Theorem~\ref{thm:cnn_thm}), and neural network with skip connections (Theorem~\ref{thm:sc_thm}) via performing a CP decomposition on each layer of the network (see ``CNN-Project'' in algorithm \ref{alg:cnn_project}, and ``TNN-Project'' in algorithm \ref{alg:tfc_project}). For the extensions to hold, we only need to assume the weight matrices/tensors of the given neural network has some CP-decomposition with no reconstruction error; this is a mild assumption as we can increase the number of components needed to obtain such a CP decomposition. This practical concern prompts for the development of a simple layer-wise structure which we call \ourNNLong (\ourNN):

While the theoretical analysis works for any network, it is not straightforward to calculate the generalization bound on a deep and large network since during the calculation, an explicit tensor decomposition procedure has to be used (see ``CNN-Project'' in algorithm \ref{alg:cnn_project}, and ``TNN-Project'' in algorithm \ref{alg:tfc_project}). This practical concern prompts for the development of a simple layer-wise structure which we call \ourNNLong (\ourNN):

\begin{definition} [\ourNN]\label{def:cpl}
  A \textit{\ourNNLong} 
  represents a given $N$-order weight tensor $\mytensor{K} \in \Rbb^{d_0 \times d_1 \times \cdots \times d_N}$ with $R$ sets of components denoted by $\Big( \lambda^{(r)}, \{\myvector{v}^{(r)}_j\}_{j=1}^{N}\Big)_{r=1}^R$ where 
  $\myvector{v}^{(r)}_j$ is a vector in $\Rbb^{d_j}$ with $l_2$ norm equal to 1. To be more specific, $\mytensor{K} = \sum_{r=1}^{R} \lambda^{(r)} \myvector{v}^{(r)}_1 \otimes \cdots \otimes \myvector{v}^{(r)}_N$.
 
  \textit{Remark.} In a \ourNNLong, $R$ denotes the number of components and $\{\lambda^{(r)}\}_{r=1}^R$ denotes the CP spectrum of this layer.
 \end{definition}

Our proposed \ourNNlong re-parametrize the networks' weights such that a CP-decomposed form can be learned easily in an end-to-end fashion. 
We demonstrate by experiments that \ourNNlong helps the network to earn a low-rank structure more easily, and thus helps with compression. This low-rankness also in return leads to a better generalization bound. 
In short, our theory results in a practical method, which we show to be of great practical and theoretical use.



==> proofs/cnn_helper_lemma_2.tex <==
\begin{proof} (of Lemma~\ref{lem:cnn_helper_lemma_2}) 
%According to Theorem~\ref{thm:cnn_fft_thm},

We know by construction, $\origcnn(\mytensor{\tinput}) = \mytensor{\tinput}^{(n+1)}$ and $\hat{\origcnn}(\mytensor{\tinput} )= \hat{\mytensor{\tinput}}^{(n+1)}$, we can just show $\fronorm{ \mytensor{\tinput}^{(n+1)} - \hat{\mytensor{\tinput}}^{(n+1)} }$ satisfies the above inequality, and we will prove this by induction. Notice

\textbf{Induction Hypothesis:} For any layer $m > 0$, $\fronorm{\mytensor{\tinput}^{(m)} - \hat{\mytensor{\tinput}}^{(m)}} \leq \sqrt{\sum_{k=1}^{m-1}\frac{(2^{m-k}\nb^{(k)})^2\cfr^{(k)}}{(\lc^{(k)})^2\fronorm{\cnnweight^{(k)}}^2}\prod_{l=k+1}^{m-1}\frac{(\tf^{(l)})^2\cf^{(l)}}{(\lc^{(l)})^2}} \fronorm{ \mytensor{\tinput}^{(m)} }$

\textbf{Base case:} when $m=1$, the above inequality hold trivially as $\mytensor{\tinput}^{(1)} = \hat{\mytensor{\tinput}}^{(1)}$ as we cannot modify the input, and the RHS is always $\geq 0$. 

\textbf{Inductive Step:} Now we assume show that the induction hypothesis is true for all $m$, let us look what happens at layer $m+1$.  As we assume perfect recovery in each layer, $\forall k$, $\{\hat{\lambda}_{r}^{(m)}, \hat{a}_{r}^{(m)}, \hat{b}_{r}^{(m)}, \hat{c}_{r}^{(m)}, \hat{d}_{r}^{(m)}\}_{r=1}^{\hat{R}^{(m)}} = \{\lambda_{r}^{(m)}, a_{r}^{(m)}, b_{r}^{(m)}, c_{r}^{(m)}, d_{r}^{(m)}\}_{r=1}^{\hat{R}^{(m)}}$, 

%We first bound $\fronorm{\tOut^{(k)}-\hat{\tOut}^{(k)}}$. According to Lemma XXX (FT is linear and perserves norm), 

\begin{equation*}
\begin{split}
\MoveEqLeft \fronorm{\mytensor{\tinput}^{(m+1)} - \hat{\mytensor{\tinput}}^{(m+1)}}^2 \\
&= \fronorm{\relu{\mytensor{\tOut}^{(m)}} - \relu{\hat{\mytensor{\tOut}}^{(m)}}}^2 \\
&\leq \fronorm{\fftYm-\fftHYm}^2 \\
&= \sum_{f,g,j}\absbig{[\fftYm]_{fgj}-[\fftHYm]_{fgj}}^2
\end{split}
\end{equation*}
the second equation holds because Fourier transformation preserves Frobenius norm.

Since
\begin{equation*}
\begin{split}
\MoveEqLeft{}
[\fftYm]_{fgj}-[\fftHYm]_{fgj}\\
&= \sum_i[\fftXm]_{fgi}[\fftMm]_{ijfg}-\sum_i[\fftHXm]_{fgi}[\fftHMm]_{ijfg}\\
&= \sum_i \big([\fftXm]_{fgi}-[\fftHXm]_{fgi}\big)\sum_{r=1}^{\hat{R}^{(m)}}\lambda_r^{(m)}a_{ri}^{(m)}b_{rj}^{(m)}\fftCm_{fg}
+\sum_i[\fftXm]_{fgi}\sum_{r=\hat{R}^{(m)}+1}^{R^{(m)}}\lambda_r^{(m)}a_{ri}^{(m)}b_{rj}^{(m)}\fftCm_{fg}
\end{split}
\end{equation*}

Let $\alpha=\sum_i\big([\fftXm]_{fgi}-[\fftHXm]_{fgi}\big)\sum_{r=1}^{\hat{R^{(m)}}}\lambda_r^{(m)}a_{ri}^{(m)}b_{rj}^{(m)}\fftCm_{fg}$, \\
and $\beta=\sum_i[\fftXm]_{fgi}\sum_{r=\hat{R}^{(m)}+1}^{R^{(m)}}\lambda_r^{(m)}a_{ri}^{(m)}b_{rj}^{(m)}\fftCm_{fg}$, then

\begin{equation*}
\begin{split}
\fronorm{\mytensor{\tinput}^{(m+1)} - \hat{\mytensor{\tinput}}^{(m+1)}}^2
&\leq \sum_{f,g,j}(\alpha+\beta)^2 \\
&\leq \sum_{f,g,j}\big(2(\alpha^2+\beta^2)\big) \\
&=2(\sum_{f,g,j}\alpha^2+\sum_{f,g,j}\beta^2)
\end{split}
\end{equation*}

So we can bound $\sum_{f,g,j}\alpha^2$ and $\sum_{f,g,j}\beta^2$ separately.

\hypertarget{bound_alpha}{\textbf{Bound $\sum_{f,g,j}\alpha^2$:}}
% \jlcomment{you can use $\big( \Big( \bigg( \Bigg($ to make the equations look nicer}
% \jlcomment{the 4th line missed a square, should be $(\sum_{r=1}^{\hat{R}{(m)}}\lambda_r^{(m)}b_{rj}^{(m)}\fftCm_{fg})^2$}
\begin{equation*}
\begin{split}
\sum_{f,g,j}\alpha^2
&= \sum_{f,g,j}\Big(\sum_i\big([\fftXm]_{fgi}-[\fftHXm]_{fgi}\big)\sum_{r=1}^{\hat{R}{(m)}}\lambda_r^{(m)}a_{ri}^{(m)}b_{rj}^{(m)}\fftCm_{fg}\Big)^2 \\
&= \sum_{f,g,j}\Big(\sum_{r=1}^{\hat{R}{(m)}}\lambda_r^{(m)}b_{rj}^{(m)}\fftCm_{fg}\sum_i\big([\fftXm]_{fgi}-[\fftHXm]_{fgi}\big)a_{ri}^{(m)}\Big)^2 \\
&\leq \sum_{f,g,j}\Bigg(\sum_{r=1}^{\hat{R}{(m)}}\lambda_r^{(m)}b_{rj}^{(m)}\fftCm_{fg}\sqrt{\bigg(\sum_i \absbig{[\fftXm]_{fgi}-[\fftHXm]_{fgi}}^2\bigg)\bigg(\sum_i(a_{ri}^{(m)})^2\bigg)}\Bigg)^2 \\
&=\sum_{f,g,j} \bigg(\sum_{r=1}^{\hat{R}{(m)}}\lambda_r^{(m)}b_{rj}^{(m)}\fftCm_{fg}\bigg)^2\bigg(\sum_i \absbig{[\fftXm]_{fgi}-[\fftHXm]_{fgi}}^2\bigg) \\ 
&\leq \sum_{f,g,j}\bigg(\sum_{r=1}^{\hat{R}{(m)}}(\lambda_r^{(m)})^2(b_{rj}^{(m)})^2\bigg)\bigg(\sum_{r=1}^{\hat{R}{(m)}}\absbig{\fftCm_{fg}}^2\bigg)\bigg(\sum_i \absbig{[\fftXm]_{fgi}-[\fftHXm]_{fgi}}^2\bigg) \\
&= \sum_{r=1}^{\hat{R}{(m)}}(\lambda_r^{(m)})^2\Bigg(\sum_{r=1}^{\hat{R}{(m)}}\sum_{f,g} \absbig{\fftCm_{fg}}^2\bigg(\sum_i\absbig{[\fftXm]_{fgi}-[\fftHXm]_{fgi}}^2\bigg)\Bigg) \\
&\leq \big(\sum_{r=1}^{\hat{R}{(m)}}(\lambda_r^{(m)})^2\big)\bigg(\sum_{r=1}^{\hat{R}{(m)}}\max_{f,g}\sum_i\absbig{[\fftXm]_{fgi}-[\fftHXm]_{fgi}}^2\bigg) \\
&\leq (\tf^{(m)})^2 \fronorm{\cnnweight^{(m)}}^2 \cf^{(m)} \fronorm{\fftXm-\fftHXm}^2\\
&= (\tf^{(m)})^2 \fronorm{\cnnweight^{(m)}}^2 \cf^{(m)} \fronorm{\mytensor{\tinput}^{(m)}-\hat{\mytensor{\tinput}}^{(m)}}^2\\
&\leq (\tf^{(m)})^2 \fronorm{\cnnweight^{(m)}}^2 \cf^{(m)} \Big(\sum_{k=1}^{m-1}\frac{2^{m-k}(\nb^{(k)})^2\cfr^{(k)}}{(\lc^{(k)})^2\fronorm{\cnnweight^{(k)}}^2}\prod_{l=k+1}^{m-1}\frac{(\tf^{(l)})^2\cf^{(l)}}{(\lc^{(l)})^2}\Big) \fronorm{\mytensor{\tinput}^{(m)}}^2 \\
&\leq (\tf^{(m)})^2 \fronorm{\cnnweight^{(m)}}^2 \cf^{(m)} \Big(\sum_{k=1}^{m-1}\frac{2^{m-k}(\nb^{(k)})^2\cfr^{(k)}}{(\lc^{(k)})^2\fronorm{\cnnweight^{(k)}}^2}\prod_{l=k+1}^{m-1}\frac{(\tf^{(l)})^2\cf^{(l)}}{(\lc^{(l)})^2}\Big) \frac{\fronorm{\mytensor{\tinput}^{(m+1)}}^2}{(\lc^{(m)})^2\fronorm{\cnnweight^{(m)}}^2} \\
&= \Big(\sum_{k=1}^{m-1}\frac{2^{m-k}(\nb^{(k)})^2\cfr^{(k)}}{(\lc^{(k)})^2\fronorm{\cnnweight^{(k)}}^2}\prod_{l=k+1}^{m}\frac{(\tf^{(l)})^2\cf^{(l)}}{(\lc^{(l)})^2}\Big)\fronorm{\mytensor{\tinput}^{(m+1)}}^2
\end{split}
\end{equation*}

\hypertarget{bound_beta}{\textbf{Bound $\sum_{f,g,j}\beta^2$:}}


\begin{equation*}
\begin{split}
\sum_{f,g,j}\beta^2
&= \sum_{f,g,j}\big(\sum_i[\fftXm]_{fgi}\sum_{r=\hat{R}^{(m)}+1}^{R^{(m)}}\lambda_r^{(m)}a_{ri}^{(m)}b_{rj}^{(m)}\fftCm_{fg}\big)^2 \\
&\leq \sum_{f,g,j}\bigg(\sqrt{\sum_i\big([\fftXm]_{fgi}\big)^2}\sum_{r=\hat{R}^{(m)}+1}^{R^{(m)}}\lambda_r^{(m)}b_{rj}^{(m)}\fftCm_{fg}\bigg)^2 \\
&\leq \sum_{r=\hat{R}^{(m)}+1}^{R^{(m)}}(\lambda_r^{(m)})^2\sum_j(b_{rj}^{(m)})^2\sum_{r=\hat{R}^{(m)}+1}^{R^{(m)}}\sum_{f,g} \absbig{\fftCm_{fg}}^2\sum_i \absbig{[\fftXm]_{fgi}}^2 \\
&\leq \sum_{r=\hat{R}^{(m)}+1}^{R^{(m)}}(\lambda_r^{(m)})^2\sum_{r=\hat{R}^{(m)}+1}^{R^{(m)}}\max_{f,g}\sum_i\absbig{[\fftXm]_{fgi}}^2 \\
&\leq (\nb^{(m)})^2\cfr^{(m)}\fronorm{\fftXm}^2 \\
&= (\nb^{(m)})^2\cfr^{(m)}\fronorm{\mytensor{\tinput}^{(m)}}^2 \\
&\leq (\nb^{(m)})^2\cfr^{(m)}\frac{\fronorm{\mytensor{\tinput}^{(m+1)}}^2}{(\lc^{(m)})^2\fronorm{\cnnweight^{(m)}}^2}
\end{split}
\end{equation*}


Combining $\sum_{f,g,j}\alpha^2$ and $\sum_{f,g,j}\beta^2$, we have
\begin{equation*}
\begin{split}
\MoveEqLeft \fronorm{\mytensor{\tinput}^{(m+1)} - \hat{\mytensor{\tinput}}^{(m+1)}}^2 \\
&\leq 2\Big(\sum_{k=1}^{m-1}\frac{2^{m-k}(\nb^{(k)})^2\cfr^{(k)}}{(\lc^{(k)})^2\fronorm{\cnnweight^{(k)}}^2}\prod_{l=k+1}^{m}\frac{(\tf^{(l)})^2\cf^{(l)}}{(\lc^{(l)})^2}+\frac{(\nb^{(m)})^2\cfr^{(m)}}{(\lc^{(m)})^2\fronorm{\cnnweight^{(m)}}^2}\Big)\fronorm{\mytensor{\tinput}^{(m+1)}}^2 \\
&= \Big(\sum_{k=1}^{m-1}\frac{2^{m-k+1}(\nb^{(k)})^2\cfr^{(k)}}{(\lc^{(k)})^2\fronorm{\cnnweight^{(k)}}^2}\prod_{l=k+1}^{m}\frac{(\tf^{(l)})^2\cf^{(l)}}{(\lc^{(l)})^2}+\frac{2(\nb^{(m)})^2\cfr^{(m)}}{(\lc^{(m)})^2\fronorm{\cnnweight^{(m)}}^2}\prod_{l=m+1}^{m}\frac{(\tf^{(l)})^2\cf^{(l)}}{(\lc^{(l)})^2}\Big)\fronorm{\mytensor{\tinput}^{(m+1)}}^2 \\
&= \Big(\sum_{k=1}^{m}\frac{(2^{m-k+1}\nb^{(k)})^2\cfr^{(k)}}{(\lc^{(k)})^2\fronorm{\cnnweight^{(k)}}^2}\prod_{l=k+1}^{m}\frac{(\tf^{(l)})^2\cf^{(l)}}{(\lc^{(l)})^2}\Big)\fronorm{\mytensor{\tinput}^{(m+1)}}^2
\end{split}
\end{equation*}


\end{proof}

==> proofs/cnn_lemma.tex <==
\begin{proof} (of Lemma~\ref{lem:cnn_lemma}) 
Based on the assumptions in section \ref{sec:setup}, the $\{\hat{R}^{(k)} \}_{k=1}^{n}$ returned by Algorithm~\ref{alg:find_best_rank_cnn} will satisfy: 
\begin{itemize}
\item $\forall k, \hat{R}^{(k)} \leq R^{(k)}$
\item $\forall k, \sqrt{(\nb^{(k)})^2 \cfr^{(k)} \Pi_{i=k+1}^{n} (\tf^{(i)})^2 \cf^{(i)}  }\leq \frac{\epsilon}{\sqrt{n2^n}}\sqrt{\fronorm{\cnnweight^{(k)}}^2 \Pi_{i=k}^n (\lc^{(i)})^2 }$
\end{itemize}

Thus, 
$$\sqrt{\sum_{k=1}^n\frac{2^{n-k+1}(\nb^{(k)})^2\cfr^{(k)}}{(\lc^{(k)})^2\fronorm{\cnnweight^{(k)}}^2}\prod_{l=k+1}^n\frac{(\tf^{(l)})^2\cf^{(l)}}{(\lc^{(l)})^2}} \leq \epsilon$$
% \jlcomment{I think the RHS of the above equation should just be $\epsilon$?}
 Then by lemma~\ref{lem:cnn_helper_lemma_2}, 
 $$\fronorm{\origcnn(\mytensor{\tinput}) -  \hat{\origcnn}(\mytensor{\tinput})} \leq \epsilon \fronorm{\origcnn(\mytensor{\tinput})}$$
\end{proof}

==> proofs/tensor_fronorm.tex <==
\begin{proof} (of Proposition~\ref{prop:tensor_fronorm}) Since $R \leq d_p, R \leq d_q$ with $p < q$, we can flatten $\mytensor{Q}$ into a matrix $\mymatrix{Q}$ by vectorizing the tensors $(\mymatrix{U_1})_i \otimes \cdots \otimes (\mymatrix{U_p})_i$ and $(\mymatrix{U_{p+1}})_i \otimes \cdots \otimes (\mymatrix{U_m})_i$ for each $i$. Let $\myvector{u_i} := vec((\mymatrix{U_1})_i \otimes \cdots \otimes (\mymatrix{U_p})_i)$ and $\myvector{v_i} = vec((\mymatrix{U_{p+1}})_i \otimes \cdots \otimes (\mymatrix{U_m})_i)$. Then $\mymatrix{Q} = \sum_{i=1}^R \lambda_i u_i \otimes v_i$. Notice that $\forall i \neq j$, 
%
\begin{equation*}
\begin{split}
\inp{\myvector{u_i} }{\myvector{u_j}} &= \sum_{k_1 \in [d_1]} \cdots \sum_{k_p \in [d_p]} [(\mymatrix{U_1})_i ]_{k_1} [(\mymatrix{U_1})_j ]_{k_1} 
%\\&\quad 
\times \cdots \times [(\mymatrix{U_p})_i]_{k_p}[(\mymatrix{U_p})_j]_{k_p}  \\
&= \sum_{k_p \in [d_p]} [(\mymatrix{U_p})_i]_{k_p}[(\mymatrix{U_p})_j]_{k_p}  
%\\&\quad 
\times \sum_{k_1 \in [d_1]} \cdots \sum_{k_{p-1} \in [d_{p-1}]} [(\mymatrix{U_1})_i ]_{k_1} [(\mymatrix{U_1})_j]_{k_1}  
%\\&\quad 
\times \cdots \times [(\mymatrix{U_{p-1}})_i]_{k_{p-1}}[(\mymatrix{U_{p-1}})_j]_{k_{p-1}}  \\
&= 0 \times  \sum_{k_1 \in [d_1]} \cdots \sum_{k_{p-1} \in [d_{p-1}]} [(\mymatrix{U_1})_i ]_{k_1} [(\mymatrix{U_1})_i ]_{k_1}   \times \cdots \times [(\mymatrix{U_{p-1}})_i]_{k_{p-1}}[(\mymatrix{U_{p-1}})_j]_{k_{p-1}} \\
& = 0 
\end{split}
\end{equation*}

Similarly, we can show $\forall i \neq j$, $\inp{u_i}{u_j} = 0$ as well. Moreover, notice that for any two vectors $\myvector{a}, \myvector{a}$, if $\norm{\myvector{a}} = \norm{\myvector{b}} = 1$, $\fronorm{a \otimes b} = \sqrt{\Tr( (\myvector{a} \myvector{b}^\top)^\top (\myvector{a} \myvector{b}^\top)} = \sqrt{\Tr (\myvector{b} \myvector{a}^\top \myvector{a} \myvector{b}^\top)} = \sqrt{\Tr (\myvector{b} \myvector{b}^\top)}  = 1$. This can also be extend to the outer product of more vectors: $\forall i$ 
%
\begin{equation*}
\begin{split}
\norm{\myvector{u_i}}^2 &= \sum_{k_1 \in [d_1]} \cdots \sum_{k_p \in [d_p]} [(\mymatrix{U_1})_i ]_{k_1}^2  \times \cdots \times [(\mymatrix{U_p})_i]_{k_p}^2 \\
&= \sum_{k_1 \in [d_1]} [(\mymatrix{U_1})_i ]_{k_1}^2 \sum_{k_2 \in [d_2]} [(\mymatrix{U_2})_i ]_{k_2}^2 \cdots \sum_{k_p \in [d_p]} [(\mymatrix{U_p})_i]_{k_p}^2  \\
&= 1 \times \cdots \times 1  = 1 \\
\end{split}
\end{equation*}
Similarly, $\forall i, \norm{\myvector{v_i}} = 1$ as well.

Then $\sum_{i=1}^R \lambda_i u_i \otimes v_i$ is a SVD of $\mymatrix{Q}$ and $\{\lambda_i\}_{i=1}^R$ are singular values of $\mymatrix{Q}$. Thus, $\fronorm{\mytensor{Q}} = \fronorm{\mymatrix{Q}} = \sqrt{\sum_{i=1}^R \lambda_i^2}$.
\end{proof}

